A Fast and Flat Federated Learning Method via Weighted Momentum and Sharpness-Aware Minimization

In federated learning (FL), models must \emph{converge quickly} under tight communication budgets while \emph{generalizing} across non-IID client distributions. These twin requirements have naturally led to two widely used techniques: client/server \emph{momentum} to accelerate progress, and \emph{sharpness-aware minimization} (SAM) to prefer flat solutions. However, simply combining momentum and SAM leaves two structural issues unresolved in non-IID FL. We identify and formalize two failure modes: \emph{local-global curvature misalignment} (local SAM directions need not reflect the global loss geometry) and \emph{momentum-echo oscillation} (late-stage instability caused by accumulated momentum). To our knowledge, these failure modes have not been jointly articulated and addressed in the FL literature. We propose \textbf{FedWMSAM} to address both failure modes. First, we construct a momentum-guided global perturbation from server-aggregated momentum to align clients' SAM directions with the global descent geometry, enabling a \emph{single-backprop} SAM approximation that preserves efficiency. Second, we couple momentum and SAM via a cosine-similarity adaptive rule, yielding an early-momentum, late-SAM two-phase training schedule. We provide a non-IID convergence bound that \emph{explicitly models the perturbation-induced variance} $\sigma_\rho^2=\sigma^2+(L\rho)^2$ and its dependence on $(S, K, R, N)$ on the theory side. We conduct extensive experiments on multiple datasets and model architectures, and the results validate the effectiveness, adaptability, and robustness of our method, demonstrating its superiority in addressing the optimization challenges of Federated Learning. Our code is available at https://github.com/Huang-Yongzhi/NeurlPS_FedWMSAM.

==> content/motivation.tex <==
%% 中文注释：以下是“Motivation”部分的示例大纲整理，采用段落式叙述。我们根据你提供的动机要点，组织成约四段，紧扣动量 vs. SAM 的优缺点对比、联邦SAM的核心难点、已有方法分类及不足、以及引出个性化动量+SAM 的方法思路。若需配图与表格，可在相应位置插入引用（如 “Figure 1” / “Table 1”），并在文中简要提及。



\begin{figure}[h!tbp]
 \vspace{-1.0em}
    \centering
    \hspace{-2.0em}
    \begin{subfigure}[b]{0.48\linewidth}
        \centering
        \includegraphics[width=1.3\linewidth]{graph/compare.png}
        \caption{Momentum vs SAM in FL}
        \label{fig:compare}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\linewidth}
        \centering
        \includegraphics[width=\linewidth]{graph/core.png}
        \caption{The core of SAMs}
        \label{fig:core}
    \end{subfigure}
    \caption{Illustration of motivation.}
    \vspace{-1.0em}
\end{figure}


\section{Motivation}
% Federated learning (FL) inherently faces two dilemmas when dealing with non-IID data: 
% how to converge fast and how to achieve strong final accuracy. On one hand, momentum-based approaches are known to accelerate training in the early stages by reusing historical gradient directions; however, they often exhibit limited performance in later stages, leading to persistent oscillations. On the other hand, SAM-based strategies typically converge to flatter minima and yield better generalization but converge relative slowly in the early epochs. 

To achieve the \textit{fast and flat} training goal, we first analyze the characteristics of momentum-based and SAM-based methods. As shown in Figure~\ref{fig:compare}, the Momentum-based method in the red line converges quickly in the early stages, but later performance fluctuates significantly and cannot further improve. In contrast, the SAM-based method in the green line has slower convergence in the beginning but steadily improves in the later stages and achieves higher accuracy.




% As shown by a simple comparison of pure momentum vs.\ pure SAM in FL (see Figure~\ref{fig:performance}), 
% one observes that momentum methods enjoy rapid initial gains yet plateau sooner, whereas SAM methods require more time to stabilize but eventually surpass in final performance.
Some methodologies, such as ~\citep{qu2022generalized}, have sought to integrate momentum and SAM to harness the advantages of both techniques. However, as elaborated in Section~\ref{section:Experiment}, a straightforward combination of momentum and SAM does not constitute a sufficient solution. Such a limitation underscores the need to propose a more thoroughly integrated approach.

Because even the benefit of generalization for applying SAM, FL triggers a core dilemma: SAM relies on perturbations computed from local data to locate "flatter" regi. Yet, in federated scenarios, each client's model and data distribution deviate from the true global model and distribution. Consequently, the local perturbation often fails to reflect the genuine global flatness, exacerbating the gap between local minima and the true global optimum, as we illustrated in ~\ref{fig:core}. This issue worsens as data heterogeneity grows and local steps increase~\citep{fan2024locally}. Hence, any FL method aiming to exploit SAM must simultaneously \textbf{(a) align the local model with the global model} and \textbf{(b) estimate the global perturbation locally}.

\begin{table*}[htbp]
\centering
\caption{Federated SAM approaches on the local-global model discrepancy, local perturbations for global objectives, communication costs (downlink/uplink), backward passes, and local storage overhead.}
% \caption{Comparison of federated SAM approaches regarding whether they reduce local--global model discrepancy, how they enable local perturbations to capture global objectives, their communication cost (downlink/uplink), number of backward passes, and local storage overhead.}
 \vspace{-1.0em}
\label{tab:fed_sam_compare}
\vspace{6pt}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccc}
\hline
\textbf{Method} & \textbf{Model Alignment} & \textbf{Global Perturbation} & \textbf{Downlink} & \textbf{Uplink} & \textbf{BP Passes} & \textbf{Local Storage} \\
\hline
\textbf{FedSAM}       & None (FedAvg)         & None                           & 1$\times$ & 1$\times$ & 2$\times$ & 1$\times$ \\
\textbf{MoFedSAM}     & Momentum (FedCM)      & None                           & 2$\times$ & 1$\times$ & 2$\times$ & 2$\times$ \\
\textbf{FedGAMMA}     & Local corr.~$c$ (Scaffold) & None                           & 2$\times$ & 1$\times$ & 2$\times$ & 3$\times$ \\
\textbf{FedSMOO}      & Reg.~term (FedDyn)    & Reg.~term                      & 3$\times$ & 2$\times$ & 2$\times$ & 4$\times$ \\
\textbf{FedLESAM}(-S/-D) & None / Local corr.~$c$ / reg.~term & Historical estimate             & 1$\times$/2$\times$/2$\times$ & 1$\times$ & 1$\times$ & 2$\times$/4$\times$/4$\times$ \\
\textbf{FedWMSAM} (ours) & Personalized momentum  & Momentum-based estimate   & 2$\times$ & 1$\times$ & 1$\times$ & 2$\times$ \\
\hline
\end{tabular}%
}
\end{table*}

We categorize existing Federated SAM approaches according to their model alignment and global perturbation processes, as shown in Table~\ref{tab:fed_sam_compare}. We also further analyze their communication, computation, and storage costs.
By adopting SAM directly, FedSAM fails to bridge the gap between local and global models, leading to misaligned perturbations. Similarly, approaches such as MoFedSAM and FedGAMMA use momentum or gradient corrections to reduce this discrepancy, yet still do not fully address how local perturbations might diverge from the global landscape, especially in highly heterogeneous settings.

Another problem is the gap between local and global landscapes. FedSMOO integrates a FedDyn-like regularization that can align both models and perturbations, but at the cost of increased storage and communication overhead. FedLESAM uses a unified "global" perturbation, typically based on the previous global gradient, but this may not adequately adapt to the landscape of different clients.

To address these issues, we propose a method that integrates momentum and SAM in a more profound way in federated learning. By injecting a personalized momentum mechanism (inspired by FedCM momentum~\citep{xu2021fedcm} and SCAFFOLD correction~\citep{karimireddy2020scaffold}) into the SAM framework, we enable each client to adapt its momentum term to its local bias. Additionally, inspired by FedLESAM~\citep{fan2024locally}, we recognize that the momentum's global information can assist local clients in better estimating the global perturbation, enabling more effective exploration of global flat minima while reducing the computational cost of perturbation estimation. Furthermore, by estimating the current training stage based on the discrepancy between momentum and the actual gradient, we dynamically balance the contributions of momentum and SAM during local training, cleverly leveraging the strengths of both techniques.


